LTL Reactive Synthesis with a Few Hints

We study a variant of the problem of synthesizing Mealy machines that enforce LTL specifications against all possible behaviours of the environment including hostile ones. In the variant studied here, the user provides the high level LTL specification {\phi} of the system to design, and a set E of examples of executions that the solution must produce. Our synthesis algorithm works in two phases. First, it generalizes the decisions taken along the examples E using tailored extensions of automata learning algorithms. This phase generalizes the user-provided examples in E while preserving realizability of {\phi}. Second, the algorithm turns the (usually) incomplete Mealy machine obtained by the learning phase into a complete Mealy machine that realizes {\phi}. The examples are used to guide the synthesis procedure. We provide a completeness result that shows that our procedure can learn any Mealy machine M that realizes {\phi} with a small (polynomial) set of examples. We also show that our problem, that generalizes the classical LTL synthesis problem (i.e. when E = {\emptyset}), matches its worst-case complexity. The additional cost of learning from E is even polynomial in the size of E and in the size of a symbolic representation of solutions that realize {\phi}. This symbolic representation is computed by the synthesis algorithm implemented in Acacia-Bonzai when solving the plain LTL synthesis problem. We illustrate the practical interest of our approach on a set of examples.

==> commentedText.tex <==

% % % % % % The realizability problem can also be seen as a two-player infinite duration game. In this game, the role of the system is played by Player~1 and the role of the environment is played by Player~2. This game is played for any infinite number of rounds. In each round, Player~2 (the environment) chooses $\inp \in \inputs$, and Player~2 (the system) reacts by choosing $\out \in \outputs$. By interacting during $\omega$ rounds, the two players form an infinite words $w=(\inp_0,\out_0)(\inp_1,\out_2) \dots (\inp_n,\out_n)\dots$ that is called the outcome of the game. Given a specification $\mathcal{S}$, this outcome is winning for Player~1 (the system) if $w \in \mathcal{S}$, otherwise it is winning for Player~2. In this game, the two players are playing strategies. A strategy for Player~1 is a function $\lambda_1 : (\inputs \times \outputs)^* \cdot \inputs \rightarrow \outputs$ and a strategy for Player~2 is a function $\lambda_1 : (\inputs \times \outputs)^* \rightarrow \inputs$. When two such strategies $\lambda_1,\lambda_2$ are fixed, they define a unique outcome defined and noted as follows:
% $${\sf Out}(\lambda_1,\lambda_2)=(\inp_0,\out_0)(\inp_1,\out_2) \dots (\inp_n,\out_n)\dots$$ 
% \noindent
% where $\inp_0=\lambda_2(\epsilon)$, where $\epsilon$ denotes the empty word, $\out_0=\lambda_1(\inp_0)$, and for all $i >0$:
% $$\inp_i=\lambda_2((\inp_0,\out_0)(\inp_1,\out_2) \dots (\inp_{i-1},\out_{i-1}))$$ $$\out_i=\lambda_1((\inp_0,\out_0)(\inp_1,\out_2) \dots (\inp_{i-1},\out_{i-1})\cdot \inp_{i}).$$

% When the specification is regular, it is well known that finite memory strategies suffices. Those finite memory strategies can be represented by Mealy machine. 
% \marginpar{Move the abstract realizability problem up ?}

% % % \paragraph{Two-player zero-sum games played on graphs} Games played on a graph is one of the fundamental tool to solve the  problem. While the classical procedure to solve the LTL realizability problem relies on the transformation of an LTL formula into a determinstic parity automaton which is then interpreted as a parity game, we will relies here on a variant of turn-based safety games. We remind their definition as well as their main properties.

% \begin{definition}
% % A two-player zero-sum safety game $G=(S,s_{{\sf init}},\Sigma_1,\Sigma_2,T,B)$ where $\spec$ is a non-empty finite set of states, $s_{{\sf init}} \in S$ is the initial state, $\Sigma_1$ is the alphabet of Player~1, $\Sigma_2$ is the alphabet of Player~2, $T: S \times \Sigma_2 \times \Sigma_1 \rightarrow S$ is the transition function, and $B \subseteq S$ is a set of bad states. 
% \end{definition}

% % % % A safety game on $G=(S,s_{{\sf init}},\Sigma_1,\Sigma_2,T,B)$ is played for an infinite number of rounds as follows. Each round proceeds as follows. If the game at the start of the round is in a state $s$, then Player~2 chooses some letter $\sigma_2 \in \Sigma2$, and then Player~1 reacts to $\sigma_2$ by choosing some letter $\sigma_1 \in \Sigma_1$, the state of the game is then updated to $s'=T(s,\sigma_2,\sigma_1)$, and a new round starts in $s'$. So, a play in a safety game on $G$ that starts in $s$ is the outcome of infinite number of rounds from $s$ and it is thus an infinite sequence of states $\rho=s_0 s_1 \dots s_n \dots$ with $s_0=s$. The outcome $\rho$ is winning for Player~1 if it avoids the bad states in $B$, i.e. $\forall i \geq 0 \cdot s_i \not\in B$. 

% \begin{lemma}
% % Given a safety game $G=(S,s_{{\sf init}},\Sigma_1,\Sigma_2,T,B)$, the set of positions from which Player~1 has a winning strategy to avoid $B$ can be computed in linear time in the size of $G$. From a winning state $s$, Player~1 can play a memoryless strategy.
% \end{lemma}

% The main properties of safety games that we need:
% \begin{itemize}
    % % \item those games are determined: each state is either winning for Player~1, i.e. he has a strategy to avoid $B$ no matter what is the behavior of Player~2, or Player~2 has a strategy to force a visit to $B$ no matter what Player~1 does.
    % \item memoryless strategies are sufficient for both players
    % \item we can represent any strategy of Player~1 by the set of its winning positions
    % \item ...
% \end{itemize}




% A language
% $L\subseteq (\inputs.\outputs)^*$ is called a \emph{safety
% language} if it is input-complete and prefix-closed in the following
% sense: for all $u\in L$, $\prefs(u)\cap
% (\inputs.\outputs)^*\subseteq L$. This definition  implies
% in particular that any unsafe word $u$ ($u\not\in L$) cannot be extended
% to a safe word $uv\in L$. A safety-language is
% naturally extended into a specification $\textsf{Safe}(L)$ called \emph{safety
  % specification} defined by $\textsf{Safe}(L) = \{ u\in (\inputs\outputs)^\omega\mid
% \prefs(u)\cap (\inputs\outputs)^*\subseteq
% L\}$. In this paper, we sometimes call $L$ a
% safety specification, having in mind $\textsf{Safe}(L)$.

%STATE MERGING:
%%% Given a preMealy machine $\MM =m(M,m_{\textsf{init}}, \trans)$ and a statem$m$ of $\MM$, the \emph{right-residual} of $m$ is defined as the language $\textsf{Right}^\MM_m = L((M,m,\trans))$. Given another state $m'\in M$, we say that $m$ and $m'$ are \emph{mergeable} if their right-residuals agree on their common input sequences, formally, it means that $\textsf{Right}_m\cup \textsf{Right}_{m'}$ is consistent.


%%%% Section omega-regular
\begin{comment}
For point $(3)$, we reason by induction on the number of iterations $j$, and we prove the following inductive property:
\begin{enumerate}
\item For all $j \geq 0$, for all $m \in M$, for all $q \in Q$, 
  \begin{enumerate}
      \item if $F_j(m)(q)=c$, with $0 \leq c \leq k$, then there exists a finite word $u \in (\inputs \outputs)^*$ such that $\transS^*(m_0,u) = m$, and there exists a prefix of a run $r$ in $\atm$ on $u$ that reach state $q$ and visits $c$ times the set of states $\{ q \in Q \mid d(q)=1 \}$. 
      \item if $F_j(m)(q)=k+1$ then there exists a finite word $u \in (\inputs \outputs)^*$ such that $\transS^*(m_0,u) = m$, and there exists a prefix of a run $r$ in $\atm$ on $u$ that reaches state $q$ and visits at least $k+1$ times the set of states $\{ q \in Q \mid d(q)=1 \}$.
  \end{enumerate}
\item For all $j \geq 0$, for all $m \in M$, for all $q \in Q$, if there exists $u \in (\inputs \outputs)^*$ such that the length of $u \leq 2 \times j$ and $\transS^*(m_0,u) = m$, and there exists a prefix of a run $r$ in $\atm$ on $u$ that reach state $q$ and visits at least $c$ times the set of states $\{ q \in Q \mid d(q)=1 \}$ then $F_j(m)(q) \geq c$ or $F_j(m)(q)=k+1$.
\end{enumerate}

\noindent
{\bf BASE CASE}. We consider here the case $j=0$. The only pair $m$, $q$ for which $F_0(m)(q)\not=-1$ is for $m=m_0$ and $q=q_{\sf init}$. The value $F(m_0)(q_{\sf init})$ is either $0$ if $d(q_{\sf init})=2$, or $1$ if $d(q_{\sf init})=1$. In both case, we take $u=\epsilon$, i.e. the empty word. For all possible values of $k$, it is easy to verify that $(1)(a)$ and $(1)(b)$ both hold. For condition $(2)$, we observe that the only word $u$ that can be considered in the existential quantification is the empty word $u=\epsilon$. As $\transS^*(m_0,u) = m_0$, condition $(2)$ holds by definition of $F_0$

\noindent
{\bf INDUCTIVE CASE}. Now, we consider the inductive case and we assume that conditions $(1)$ and $(2)$ hold for all $F_k$ with $0\leq k<j$, and let us show that then it holds for $j$. 

Let us recall that by definition of the sequence of labelling, we have:
$$F_j(m)=\bigsqcup_{(m_1,\inp,\out,m) \mid \Delta(m_1,\inp,\out)=m} \delta^{\mathcal{D}}(F_{j-1}(m_1),(\inp,\out)).$$
\noindent
Let us first consider the case where $F_j(m)(q)=c$ with $0 \leq c \leq k$. By definition of the sequence of labelling, we have that


Assume that in that expression, the value assigned to $q$ by $F_j$ is realized by a transition $e$ labelled with $(\inp,\out)$ from state $q_1$ to state $q$ in $\atm$. 
By induction hypothesis, we know that there exists a word $u_1 \in (\inputs \outputs)^*$, such that $\transS(m_0,u_1)=m_1$ and there is a run $r_{m_1,q_1}$ in $\atm$ on $u$ that reaches $q_1$ and visits $c$ times the set of states labelled with color $1$ in $\atm$, if $d(q)=2$ or $c-1$ visits to $c$ if $d(q)=1$. We can then construct the word $u=u_1 \cdot (\inp,\out)$ and the run $r=r_{m_1,q_1} \cdot e$. We can verify that condition $(1)(a)$ holds as required.

Let us now consider the case where $F_j(m)(q)=k+1$. Assume that in that expression, the value assigned to $q$ by $F_j$ is realized by a transition $e$ labelled with $(\inp,\out)$ and from state $q_1$ to state $q$ in $\atm$. 
By induction hypothesis, we know that there exists a word $u_1 \in (\inputs \outputs)^*$, such that $\transS(m_0,u_1)=m_1$ and there is a run $r_{m_1,q_1}$ in $\atm$ on $u$ that reaches $q_1$ and visits at least $k+1$ times the set of states labelled with color $1$ in $\atm$, if $d(q)=2$ or at least $k$ visits to states labelled with color $1$ if $d(q)=1$. For this case, we can then construct the word $u=u_1 \cdot ((\inp,\out)$ and the run $r=r_{m_1,q_1} \cdot e$. We can verify that condition $(1)(b)$ holds as required.

%condition (2)
We now turn to condition $(2)$. Let us assume that there exists a word $u \in (\inputs \outputs)^*$ of length at most $2 \times j$ such that $\transS(m_0,u)=m$ and such that there is a prefix of run $r$ of $\atm$ on $u$ that visits at least $c$ the set of states $\{ q \in Q \mid d(q)=1\}$, we need to show that $F_j(m)(q) \geq c$ if $0 \leq c \leq k$, and $F_j(m)(q) = k+1$ if $c \geq k+1$. 

As $j \geq 1$, we can decompose $u$ into $u=u_1 \cdot (\inp,\out)$. By induction hypothesis, we know that for $m_1=\transS(m_0,u_1)$, all $q_1$ reached by a prefix of run in $\atm$ on $u_1$ that visits the set of states $\{ q \in Q \mid d(q)=1\}$ at least $c'$ times, then we have $F_{j-1}(m_1)(q_1) \geq c'$ if $0 \leq c' \leq k$, and $F_{j-1}(m_1)(q_1) = k+1$ if $c' \geq k+1$. So, let us consider a run $r$ of $\atm$ on $u=u_1 \cdot (\inp,\out)$ and its prefix $r_1$ on $u_1$. Let $c$ be the number of visits to the set $\{ q \in Q \mid d(q)=1\}$ by $r$, and $c'$ the number of visits of $r_1$ to this set. We have that $c=c'$ if the last state $q$ visited by $r$ is such that $d(q)=2$, and we have that $c=c'+1$ if  the last state $q$ visited by $r$ is such that $d(q)=1$. By induction hypothesis and the definition of $F_j(m)(q)$, we have that in both cases $F_j(m)(q) \geq c$ if $0 \leq c \leq k$, and $F_j(m)(q)=k+1$ if $c \geq k+1$. 
\end{comment}
\begin{comment}

\section{LTL-specification driven state-merging and state-completion heuristics}
In this section, we speak about the different state-merging ($\sigma_G$) and state-completion ($\sigma_C$) algorithms that we have used in our tool. 
\subsection{State-merging based on closeness in counting functions}
Here, given a pre-mealy machine $\mathcal{M_0} = (M, m_{\mathsf{init}}, \Delta)$, a merge candidate state $m \in M$ and a set of candidate edges $mergeCand$ which are \textit{compatible} with $m$, we then choose an edge $e= (m,i) \to (m',o) \in mergeCand$ such that the difference (edit distance) between the counting functions the $F^*(m)$ and $F^*(m')$ obtained from the specification $\spec$ is minimal.
\begin{algorithm}[h]
\DontPrintSemicolon
\KwIn{A Pre-mealy machine $\mathcal{M_0} = (M, m_{\mathsf{init}}, \Delta)$, state $m$, set of edges $mergcand$, a specification $\spec \subseteq (\mathcal{I}\cdot\mathcal{O})^*$ given as a deterministic safety automaton}
\KwOut{Edge $e \in mergeCand$.}
\Begin{
    Compute $F^*: M \to CF(\mathcal{A}, k)$ for the specification $\spec$\;
    Choose an edge $e = (m, i) \to (m', o) \in mergeCand$ such that difference between the counting functions $F^*(m')$ and $F^*(m)$  is minimal.\;
    \Return{$m'$}
}
\caption{Merging Strategy $\sigma_G(M,m,mergeCand,\spec) )$\label{alg:sort_comp_pairs}}
\end{algorithm}
\subsection{State-merging based on smallest counting functions}
Here, given a pre-mealy machine $\mathcal{M_0} = (M, m_{\mathsf{init}}, \Delta)$, a merge candidate $m \in M$ and a set of candidate edges $mergeCand$, we return an edge $e = (m,i) \to (m', o) \in mergeCand$ such that the counting function $F*(m)$ obtained from the specification is minimal.
\begin{algorithm}[h]
\DontPrintSemicolon
\KwIn{A Pre-mealy machine $\mathcal{M_0} = (M, m_{\mathsf{init}}, \Delta)$, state $m$, set of edges $mergcand$, a specification $\spec \subseteq (\mathcal{I}\cdot\mathcal{O})^*$ given as a deterministic safety automaton}
\KwOut{Edge $e \in mergeCand$}
\Begin{
    Compute $F^*: M \to CF(\mathcal{A}, k)$ for the specification $\spec$\;
    Choose an edge $e \in mergeCand$ such that $F^*(m')$ is the smallest.\;
    \Return{$m'$}
}
\caption{Merging Strategy $\sigma_G(M,m,mergeCand,\spec) )$\label{alg:sort_comp_pairs}}
\end{algorithm}
\end{comment}

%A straighforward application of the construction defined in the previous section would give a procedure that is doubly exponential in the size of the specification $\atm$ and the set of example $E$. Indeed, the complexity of the construction is in exponential time in the size of the deterministic parity automaton for the specification, and such a automaton is in the worst-case doubly exponential in the size of the LTL formula. Here, we propose an alternative procedure with a better worst-case complexity and which is also more amenable to an efficient implementation. Our solution relies on $K$-universal co-Buchi automaton and is inspired by~\cite{} and is variant of the Safraless construction first defined in~\cite{}.
\begin{comment}
\subsection{LTL reactive synthesis via $K$-universal co-B\"uchi automaton} Given an LTL formula $\varphi$, we can construction an universal co-B\"uchi automaton $\atm$ such that $L^{\forall}(\atm)$ is exactly the set of models of the formula $\varphi$. This is summarized in the following lemma:

\begin{lemma}[LTL to Uco-BW] Given an LTL formula $\varphi$ on the alphabet $\Sigma=\inputs \times \outputs$, we can construction an universal co-B\"uchi automaton $\atm_{\varphi}$ in time and of size $2^{{\bf O}(|\varphi|)}$ on the alphabet $\Sigma$ such that $\sem{\varphi}=L^{\forall}(\atm_{\varphi})$.
\end{lemma}

The algorithms to solve the reactive synthesis problem rely on deterministic automata, and not on nondeterministic or universal                                        automata. So, a deterministic variant of $\atm_{\varphi}$ is needed. To avoid the application of constructions that remove nondeterminism from $\atm_{\varphi}$ directly, we proceed with a Safraless approach, that consists first in defining a safety subset of $L^{\forall}(\atm_{\varphi})$ which is obtained by strengthening the acceptance condition of $\atm_{\varphi}$. The correctness of this approach is justified by the following lemma and lemma~\ref{lem:k-co}:

\begin{lemma}
\label{lem:safraless}
For all LTL formula $\varphi$ on the alphabet $\Sigma=\inputs \times \outputs$, for all universal co-B\"uchi automata $\atm_{\varphi}$, such that $\sem{\varphi}=L^{\forall}(\atm_{\varphi})$, there is $K \in \mathbb{N}$ (bounded by $2^{2^{{{\bf O}(|\varphi|)}}}$) such that $\sem{\varphi}$ is realizable if and only if $L^{\forall}_K( \atm_{\varphi})$ is realizable.
\end{lemma}


  
\subsection{LTL two-phase learning algorithm}

We now describe our main algorithm for learning a Mealy machine that generalizes the examples $E$ given by the user and realize the specification $\varphi$. Our algorithm relies on the translation of $\varphi$ into a universal co-B\"uchi automaton and on the reduction to safety languages defined in the previous subsections. It reuses the procedure to generalize examples and complete preMealy machine defined in Sect.~4. The algorithm is incremental and consider increasing value $k$ as needed.

We have seen in the previous subsection how to check the $\MM$-realizability of a specification expressed as a $k$ co-B\"uchi universal automaton $\atm_k$. We know show how to extend systematically a preMealy machine $\MM$ into a full machine $\MM'$ that realizes the specification $\atm_k$ when this specification is $\MM$-realizable.




The correctness and worst-case optimality of Algo.~\ref{algo:learningLTL} is established in the proof of the following theorem.

\begin{thm}[\cite{}]\label{thm:correctnessAlgoLTL}
Given an LTL specification $\varphi$ over atomic propositions $P_{I}$ and $P_{O}$, and a finite set of examples $E \subseteq (\inputs \outpus)^*$ where $\inputs=2^{P_I}$, and $\outputs=2^{P_O}$, if there exists a Mealy machine $\MM$ such that $E \subseteq L(\MM) \subseteq \sem{\varphi}$, then Algo.~\ref{algo:learningLTL} returns a machine $\MM'$ such that $E \subseteq L(\MM') \subseteq \sem{\varphi}$, otherwise it returns {\it UNREAL}, the worst-case complexity of the algorithm is 2ExpTime.
\end{thm}
\begin{proof}
\end{proof}
\end{comment}

\begin{comment}
\paragraph{Safety game on $\mathcal{D}(\atm,k)$} Now that we have a deterministic automaton, we can solve its associated realizability problem by playing a game on it. The game is played by two players: Player~1 that represents the system and Player~2 that represents the environment. This game is played for infinitely many rounds as follows. Initially, we place a token on $f_1=q'_{{\sf init}}$ and the first round can start. As in all rounds, Player~2, the environment, first chooses some input $\inp \in \inputs$, and Player~1 reacts by choosing some output $\out \in \outputs$. The token is then moved to state $f_2=\delta'(f_1,(\inp,\out))$, and a new round is started from there. This interaction generates an infinite run $r=f_0 f_1 \dots f_n \dots$ in the automaton $\mathcal{D}(\atm,k)$, and Player~1 is the winner if for all $i \geq 0$, $d'(f_i)=2$, or equivalently if for all $i \geq 0$, for all $q \in Q$, $f_i(q) \leq k$. Otherwise, Player~2 (the environment) is the winner.

Given a counting function $f$, we say that Player~1 has a winning strategy from $f$ in the realizability game defined by $\mathcal{D}(\atm,k)$ if Player~1 has a strategy to choose his inputs from all interaction that starts in $f$ so that the token avoid for ever counting functions $f'$ such that $d'(f')=1$ (or equivalently, counting $f'$ such that $\exists q \in Q \cdot f'(q)=k+1$). This set of counting function can be computed by iterating the controller predecessor operator which is defined as follows. Given a set of counting function $F \subseteq CF(\atm,k)$, the set of {\em controllable predecessors} of $F$ for Player~1, noted $\cpre(F)$ is defined as follows:
$$\cpre(F)=\{ f \in CF(\atm,k) \mid \forall \inp \in \inputs \cdot \exists \out \in \outputs \cdot \delta'(f,(\inp,\out)) \in F \}.$$
\noindent
So, the set of controllable predecessor of $F$ is exactly the set of counting functions from which Player~1 can force to move the token to $F$, no matter what is the choice of input by Player~2.

The set of counting functions from which Player~1 can avoid unsafe counting functions for ever is then computed as the limit of the following decreasing sequence of sets: let 
$$S_0 = \{ f \in CF(\atm,k) \mid d'(f)=2 \},$$ 
\noindent
and for all $i \geq 1$, 
$$S_i=\cpre(S_{i-1}).$$ 
\noindent
We note $S^*$ the set of counting function on which this sequence stabilizes.
The following theorem states the correctness of this realizability algorithm:

\begin{thm}
The set $S^*$ contains exactly all the counting functions from which Player~1 has a winning strategy. The language $\mathcal{D}(\atm,k)$ is realizable if and only if $f_0=q'_{{\sf init}} \in S^*$.
\end{thm}

The set $S^*$ posses some interesting structure. To reveal this structure, we first define an order on the counting functions and show that the set of counting functions equipped with this order form a complete lattice.

\begin{lemma}
Let $CF(\atm,k)$ be a set of counting function and let $\preceq \subseteq CF(\atm,k)$ be such that $f_1 \preceq f_2$ if and only if $f_1(q) \leq f_2(q)$ for all $q \in Q$. The partially ordered set $(CF(\atm,k),\preceq))$ forms a complete lattice with the following least upper bound operator:
    $f_1 \sqcup f_2=f$ where $f(q)=\max(f_1(q),f_2(q))$. The maximal length of a chain in this lattice is bounded by $|Q| \times (k+2)$.
\end{lemma}

Given a set $F \subseteq CF(\atm,k)$, we say that $F$ is $\preceq$-downward closed if $\forall f,f' \in CF(\atm,k) \cdot f' \preceq f \cdot f \in F \rightarrow f' \in F$. We write $\lceil F \rceil$ for the $\preceq$-maximal elements in $F$, i.e. $\lceil F \rceil =\{ f \in F \mid \not\exists f' \in F \cdot f\not=f' \land f \preceq f' \}$. Given a set $F \subseteq CF(\atm,k)$, we define the $\preceq$-downward closure of $F$ as $\downarrow F=\{ f' \in CF(\atm,k) \mid \exists f \in F \cdot f' \preceq f \}$.
The set $S^*$ enjoins the following structure. 

\begin{lemma}
The set $S^*$ is $\preceq$-downward closed and thus the set $S^*$ can be symbolically represented using its $\preceq$-maximal elements $\lceil S^* \rceil$.
\end{lemma}

\paragraph{Checking $P$-realizability of $L^{\forall}_K(\atm_{\varphi})$ given $\lceil S^* \rceil$} We now show that given the set $\lceil S^* \rceil$ of safe maximal counting function of a specification $L^{\forall}_K(\atm_{\varphi})$, we can determine in polynomial time in the size of $\atm_{\varphi}$, $k$, and $|\lceil S^* \rceil|$, and $|P|$ if a preMealy Machine $P$ can be complete into a Mealy Machine $M$ that realizes the specification $L^{\forall}_K(\atm_{\varphi})$.

To establish this result, 


To compute the set of 

This is a crucial point for  to compute a representation of all possible winning strategy for the language defined 

way to represent all the winning strategies that realizes $L^{\forall}_K( \atm_{\varphi})$. This is done by considering the graph of {\em counting functions} that we recall here. 



\paragraph{Content}
\begin{itemize}
  \item explain how to turn LTL into larger and larger safety
    specifications (explain counting functions)
  \item prove that from an LTL spec and a set of positive examples,
    one can compute a minimal $K$ such that there is a Mealy machine
    realizing both the spec and the examples
  \item explain that the consistency test of the learning algorithm is
    costly (we can give a theorem there) and how precomputing the
    antichain is beneficial
  \item for the latter, give the fixpoint algorithm which assigns
    counting functions to a preMealy machine and prove that it runs in
    ptime. (complexity is K times size of M times size of UcoBW (number of dim of counting functions)
    
\end{itemize}
\end{comment}

